App-based saccade latency and error determination across the adult age spectrum

We aid in neurocognitive monitoring outside the hospital environment by enabling app-based measurements of visual reaction time (saccade latency) and error rate in a cohort of subjects spanning the adult age spectrum. Methods: We developed an iOS app to record subjects with the frontal camera during pro- and anti-saccade tasks. We further developed automated algorithms for measuring saccade latency and error rate that take into account the possibility that it might not always be possible to determine the eye movement from app-based recordings. Results: To measure saccade latency on a tablet, we ensured that the absolute timing error between on-screen task presentation and the camera recording is within 5 ms. We collected over 235,000 eye movements in 80 subjects ranging in age from 20 to 92 years, with 96% of recorded eye movements either declared good or directional errors. Our error detection code achieved a sensitivity of 0.97 and a specificity of 0.97. Confirming prior reports, we observed a positive correlation between saccade latency and age while the relationship between error rate and age was not significant. Finally, we observed significant intra- and inter-subject variations in saccade latency and error rate distributions, which highlights the importance of individualized tracking of these visual digital biomarkers. Conclusion and Significance: Our system and algorithms allow ubiquitous tracking of saccade latency and error rate, which opens up the possibility of quantifying patient state on a finer timescale in a broader population than previously possible.

==> cut-outs.tex <==
Accurate quantification of neurodegenerative disease progression and neurocognitive decline is an ongoing challenge that complicates efforts to understand and treat these conditions. The current gold standard are neurocognitive assessments administered through questionnaires that are qualitative and suffer from high retest variability. Thus, there is a need for a quantitative metric that can accurately track neurocognitive decline or neurodegenerative disease progression. Clinical studies have shown that saccade latency -- an eye movement measure of reaction time -- can be significantly different between healthy subjects and patients with neurodegenerative diseases. Hence, we propose and test a novel system that enables measurement of saccade latency outside of the clinical environment. Our eye-tracking algorithm (iTracker-face), a variant of a deep-learning approach that estimates gaze on mobile devices, was tailored to robustly measure saccade latency on video sequences obtained with an iPhone 6. Additionally, our model-based approach for saccade latency estimation provides a means to automatically flag eye position traces that should not be included in the analysis (AUC = 0.92). Because of the accessibility of our system, we recorded over 20,000 saccade latencies in 30 healthy subjects and discovered that there is substantial intra- and inter- subject variability in the saccade latency measurements. This variability suggests that the common approach of pooling saccade latencies to mitigate the lack of data confounds the results of a study. Our work addresses this issue by making the measurement of saccade latency more accessible through the use of consumer-grade cameras, potentially enabling individualized unobtrusive tracking of neurodegenerative disease progression.




To robustly fit a log-normal model, we first inspect the distributions of log saccade latencies. If we assume the data is log-normally distributed, these log-latency distributions should be normal distributions. However, since we assume that a saccade with latency value smaller than 80 ms may be anticipatory, log-latency values below $\log(80)$ may not follow the same normal distribution as values above. As a result, we cannot estimate the mean and standard deviation of the log-normal model by calculating the mean and standard deviation of the entire log-latency data.

To address this difficulty, we consider a probit model \cite{Bliss}, which fits normally distributed data into a linear model. It calculates the cumulative density function $F_X(x)=P(X\leq x)$ of the data $X$, and find a transformation function $g(z)$ so that $g(F_X(x))$ becomes linear. With our assumption, we then can assume that for $x\geq \log(80)$, $g(F(x))$ is linear. Since one can use the slope and the x-axis intersection of the linear model to find the mean and standard deviation of the normally distributed data, we then can apply the linear model only on log saccade latencies greater than $\log(80)$ to find the log mean and log standard deviation. With a probit model, we are able to fit a distribution on the desired portion of the data (without fitting the anticipatory data). We can express the procedures as follows:

If $X\sim \mathcal{N}(\mu,\sigma^2)$, then one can show that
\begin{equation}
\sqrt{2}{erf}^{-1}(2(F_X(x)-1))=\frac{x-\mu}{\sigma},
\end{equation}
where ${erf}^{-1}(\cdot)$ denotes the inverse of the error function, which is defined as
\begin{equation}
erf(x)=\frac{2}{\sqrt{\pi}}\int_0^x e^{-t^2}dt,
\end{equation}
and $F_X(x)$ denotes the cumulated density function of $X$.

If our y-axis is $y=g(x)=\sqrt{2}erf^{-1}(2(F_X(x)-1))$, then the relationship between $x$ and $y$ should be linear (this is the probit model). The mean of the data $X$ will be the intersection of the line with the x-axis, and the standard deviation will be the reciprocal of the slope.

A typical probit plot for a normal subject's log-saccade latency values is shown in Fig.~\ref{fig:probit}. Instead of fitting a linear line on data with log latency values above $\log(80)$, we fit a linear model on data points lying between 0.05 quantile and 0.95 quantile so that the estimated parameters will be even more robust to outliers. If the fitting line has a form of $y=ax+b$, then we estimate the mean value to be $-b/a$ and the standard deviation to be $1/a$. After the mean and the standard deviation of the log-normal model are estimated, we define the model for each distribution as the estimated log-normal model truncated at 80 ms.

\begin{figure}[b]%[thpb]
\vspace{-10pt}
      \centering
      \includegraphics[scale=0.4]{Figure/all_individual_hist.eps}
      \caption{Distribution of mean saccade latency values from 30 healthy individuals.}
      \label{fig:everyone}
   \end{figure}

%\begin{figure}[t]%[thpb]
%\vspace{-10pt}
%      \centering
%      \includegraphics[scale=0.2]{Figure/probit_example.eps}
%      \caption{The probit plot for the log-latency values of subject 001. The blue line shows the linear fit.}
%      \label{fig:probit}
%   \end{figure}


%Need to be recalculated


We also report the distribution of the mean saccade latencies across 30 subjects. The histogram in Fig.~\ref{fig:everyone} shows the distribution of the mean saccade latencies from the first recording session across all subjects, and indicates that there is a significant range in mean saccade latencies even in the healthy population.





In order to use saccade latency to track neurodegenerative disease progression, it is important to understand the intra- and inter-subject variability among healthy subjects to put into context the changes seen in patients with neurodegenerative disease. Most clinical studies~\cite{Shafiq_2003, Boxer_2012} lack a set-up that allows for multiple measurements of saccade latency. To lessen the effect of insufficient data, these studies pool the saccade latencies from healthy subjects and patients into two separate distributions: the healthy subjects distribution (Fig.~\ref{fig:everyone}) and the patient distribution. In this approach, intra- and inter-subject variability is not taken into account. 

%very few studies~\cite{multimodal} have reported repeat measurements per individual. 

In our work, we measured more than 1,200 saccade latencies in each of ten subjects (Fig.~\ref{fig:tenhist}), a significantly larger amount compared to the values reported in clinical studies, ranging from 8 -- 30 saccade latencies~\cite{Heuer_2013,Crawford_2005,Garbutt_2008,Boxer_2012}. These recordings were enabled by the accessible nature of our measurement system that allows for 120 saccade measurements in less than eight minutes. Considering the criteria to reject certain saccade latencies, we are still able to retain, on average, a sizable amount (81\%) of data per session across subjects. 

With this amount of data, we observed that saccade latency intra- and inter-subject variability is quite substantial, with mean saccade latencies ranging from 126 ms -- 173 ms and standard deviations from 24 ms -- 53 ms (Fig.~\ref{fig:tenhist}). Given the inter-subject variability, the common approach of pooling data from different subjects is not appropriate as doing so increments variability, confounding the results of a study and making it harder to draw conclusions about healthy and patient populations. Furthermore, the information regarding the distinctive shape and parameters of the individual distributions is lost when saccade latency values are pooled. As seen in Fig.~\ref{fig:tenhist}, some individuals have a tendency to make more saccades with shorter latencies (Subjects 004, 009, and 037) and others to make more saccades with longer latencies (Subjects 007, 009, 010). In combining all the data into a single distribution, these individual characteristics that have been linked to specific brain pathologies~\cite{Rivaud_1994,Pierrotdeseilligny_2003} are lost. Saccade latency intra-subject variability is also neglected when data is pooled. If instead the information regarding this variability ($\sigma$) were preserved, it could be used as a feature to assess the cognitive state of a subject. For example, some studies suggest that intra-subject variability is larger in schizophrenic patients compared to normal subjects~\cite{Theleritis_2014,Karantinos_2014}.
Our accessible, low-cost measurement system enables widespread data collection and hence avoids having to combine data from different subjects, allowing us to preserve the distinctive information in each individual saccade latency distribution.

We observed that the saccade latency distribution of the majority of the subjects may be modeled as a log-normal distribution. 
% Should we still cite this?
This observation is consistent with~\cite{Ulrich_1993}, in which neural mechanisms are discussed that might give rise to log-normally distributed reaction times. 
It might therefore be sufficient to characterize individual saccade-latency distributions using the two parameters of a log-normal distribution ($\log-\mu$ and $\log-\sigma$) and analyze how these parameters change through time. In our longitudinal analysis, however, we evaluated how the mean ($\mu$) and the standard deviation ($\sigma$) of the saccacde-latency distributions changed across time. These statistics were chosen over the mode or the median for two major reasons: (1) the mode, mean, and median tracked one another closely; and (2) clinical studies usually report the mean and standard deviation. 

% we may need to re-write this part and cite the other paper
% point out the fact that previously there seems to be some learning effects but in long term most slopes seem not to be significantly different from 0

\noindent\textit{Saccade latency measurements in healthy subjects}\\
One of our goals is to understand the nature and variability of saccade latency among normal, healthy subjects. In~\cite{Saavedra_2018}, we observed that there was a substantial amount of intra-subject variability in the mean and standard deviation of saccade latency. With only five sessions from ten subjects, it was difficult to quantify the variability in these measurements across time. To address this, we augmented our data by collecting data in ten different sessions from ten subjects. A linear model on the mean saccade latency across sessions per individual showed that the slope of this line is not significantly different from zero in six out of ten subjects. That is, although the variation in the mean and the standard deviation remain significant, both parameters seem to be stationary across time for the majority of subjects. 
Furthermore, the values of the coefficient of determination, $R^{2}$, suggests that the variability in these measurements cannot be exclusively explained by the number of recorded sessions. For example, tiredness can be another factor that introduces the variability. More work is needed to elucidate and isolate these other effects. 

%One of the goals of our work is elucidating whether repeat measurements of saccade latency can be used to assess neurocognitve decline. Therefore, it is important to understand the behavior and variability of saccade latency in healthy subjects. To aid our understanding, we took multiple measurements of saccade latency per individual across days and analyzed the patterns in these measurements. The recording sessions are sequential but were not necessarily taken on consecutive days. Ultimately, the mean and standard deviation of the saccade-latency distributions were analyzed as a function of the individual recording sessions. Fig.~\ref{fig:longt} shows that for each subject, the mean saccade latency and the standard deviation change across recording sessions. A linear model on the mean saccade latencies across recording sessions accounted for 1\% to 84\% of the variability in the measurements. This suggests that although the mean saccade latencies varies with the number of recording sessions, there are other factors (such as tiredness or test-taking strategies) that introduce variability. To quantify the changes in these values for tracking of disease progression, we need to analyze a sufficient amount of recordings to isolate these factors. With our approach to measure saccade latency using laptop and smartphone cameras, it is promising to identify these factors while current clinical methods are too restrictive.


